Histopathological Image Classification and Vulnerability Analysis using Federated Learning

Healthcare is one of the foremost applications of machine learning (ML). Traditionally, ML models are trained by central servers, which aggregate data from various distributed devices to forecast the results for newly generated data. This is a major concern as models can access sensitive user information, which raises privacy concerns. A federated learning (FL) approach can help address this issue: A global model sends its copy to all clients who train these copies, and the clients send the updates (weights) back to it. Over time, the global model improves and becomes more accurate. Data privacy is protected during training, as it is conducted locally on the clients' devices. However, the global model is susceptible to data poisoning. We develop a privacy-preserving FL technique for a skin cancer dataset and show that the model is prone to data poisoning attacks. Ten clients train the model, but one of them intentionally introduces flipped labels as an attack. This reduces the accuracy of the global model. As the percentage of label flipping increases, there is a noticeable decrease in accuracy. We use a stochastic gradient descent optimization algorithm to find the most optimal accuracy for the model. Although FL can protect user privacy for healthcare diagnostics, it is also vulnerable to data poisoning, which must be addressed.

==> background.tex <==
ML has the potential to revolutionize many aspects of life, including healthcare, transportation, and education. Many industries and organizations now rely on ML to evaluate massive volumes of data and make predictions or decisions. However, ML frequently requires the collecting and processing of sensitive personal information, which might cause privacy concerns. Protecting the privacy of people whose data are used in the training of the models is one of the most important issues. In response to these issues, several techniques have been developed to protect privacy:

\begin{itemize}
\item \textbf{Differential privacy} This method involves incorporating noise into the data in a way that maintains privacy without compromising the accuracy of the ML model \cite{dwork2006calibrating}. Depending on the sensitivity of the data and the desired level of privacy, the amount of noise introduced is calibrated. Differential privacy offers a significant advantage by providing a verified guarantee of privacy. This means that it is possible to demonstrate mathematically that data confidentiality is maintained. Achieving a balance between privacy and accuracy can be challenging. In fact, introducing a considerable amount of noise to the data may be necessary to ensure a strong privacy guarantee.

\item \textbf{Homomorphic Encryption} With this technique, it is possible to train a machine-learning model using encrypted data without any decryption  \cite{gentry2009fully}. This can be useful when the data are sensitive and cannot be decrypted or when the data is owned by different parties who do not wish to share the information. One of the primary advantages of homomorphic encryption is that enterprises can achieve a higher data security standard without compromising business processes or the functioning of the application. These enterprises can protect data privacy while collecting intelligence from sensitive data. However, using homomorphic encryption with certain types of ML models may not be practical due to its high computational cost.

\item \textbf{Secure multiparty computation} This is a cryptographic technique that provides a protocol in which no individual can view the data of other parties during data distribution \cite{yao1982protocols}. It allows data scientists and analysts to perform private computations on distributed data without revealing them. One of the main benefits of multiparty computation is that it preserves data accessibility and confidentiality by making it easy to perform collaborative calculations without hiding any variables. Without jeopardizing precision, data confidentiality is maintained in its entirety. On the other hand, this approach generates vast quantities of random numbers, which require computational resources. Additionally, diverse server systems and storage devices can reduce the performance of multiparty computation protocols.

\item \textbf{Federated Learning}  This approach permits many parties to train a ML model without sharing their respective data \cite{mcmahan2017communication}. This can be particularly useful in situations where the data are sensitive and sharing them is not possible, or when multiple parties own the data and are unwilling to share them. In federated learning, each party trains a local model on its own data and then sends model changes to a central server, which combines the updates to form a global model. One of the primary advantages is that it enables the model to get trained on a larger dataset, as it may be trained on data from several parties. Nevertheless, due to the need for model updates to be transmitted between parties, federated learning can be slower than conventional ML methodologies.
\end{itemize}
